SIDNet: Learning Shading-aware Illumination Descriptor for Image Harmonization

Image harmonization aims at adjusting the appearance of the foreground to make it more compatible with the background. Without exploring background illumination and its effects on the foreground elements, existing works are incapable of generating a realistic foreground shading. In this paper, we decompose the image harmonization task into two sub-problems: 1) illumination estimation of the background image and 2) re-rendering of foreground objects under background illumination. Before solving these two sub-problems, we first learn a shading-aware illumination descriptor via a well-designed neural rendering framework, of which the key is a shading bases module that generates multiple shading bases from the foreground image. Then we design a background illumination estimation module to extract the illumination descriptor from the background. Finally, the Shading-aware Illumination Descriptor is used in conjunction with the neural rendering framework (SIDNet) to produce the harmonized foreground image containing a novel harmonized shading. Moreover, we construct a photo-realistic synthetic image harmonization dataset that contains numerous shading variations with image-based lighting. Extensive experiments on both synthetic and real data demonstrate the superiority of the proposed method, especially in dealing with foreground shadings.

==> Tables/AblationDepth.tex <==
\begin{table}[]
\centering
\resizebox{0.9\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{@{}l|ccc@{}}
\toprule
& fMAE$\downarrow$  & fPSNR$\uparrow$ & fSSIM$\uparrow$ \\ \midrule
Ours w/o depth                                   & 0.057 & 22.77 & 0.874 \\
Ours                         & 0.054 & 23.64 & 0.908 \\ \bottomrule
\end{tabular}
}
\caption{Effects of the depth maps.}
\label{tab:ablation_depth}
\end{table}

==> Tables/AblationGAB.tex <==
\begin{table}
\centering
\caption{Ablation study on GAB.}
%\resizebox{0.7\linewidth}{!}{
\setlength{\tabcolsep}{3mm}
\begin{tabular}{l|cc}
\hline
 & fPSNR$\uparrow$ & fSSIM$\uparrow$ \\ \hline
Shading Bases Module w/o GAB & 30.75 & 0.928 \\
Shading Bases Module &\textbf{31.35} & \textbf{0.936} \\
\hline
\end{tabular}
%}
\label{tab:ablation_GAB}
\end{table}

==> Tables/network_illum.tex <==
\begin{table}
\centering
\caption{Our illumination network architecture. We use this architecture for both the \textbf{Background Illumination Estimation Module} and  \textbf{Illumination Encoder Module}.}
\resizebox{.45\textwidth}{!}{%

\begin{tabular}{ l  c c c c c c c c }

\hline
Layers & \multicolumn{8}{c}{Parameters}  \\ 
\hline


  & \textbf{k}  & \textbf{s} & \textbf{d}  & \textbf{p} &  \textbf{chns} &  \textbf{input} &   &  \\
	\hline
	
$\text{conv3x3}_{1}$ & 3 & 1 & 1 & 1 & 3/32 & $I_{in}$ \\
$\text{conv3x3}_{2}$ & 3 & 1 & 1 & 1 & 32/32 & $\delta$($\text{conv3x3}_{1}$) \\
$\text{Pool}_{1}$ & 2 & 1 & - & 0 & 32/32 & $\delta$($\text{conv3x3}_{2}$) \\
\hline

& \textbf{k}  &  \textbf{s} & d  &   \textbf{chns} &   \textbf{n-l} &   \textbf{g-r} &   \textbf{input} \\
\hline

$\text{RDB}_{1,1}$ & 3 & 1 & 1 & 32/32 & 8 & 16 & $\text{Pool}_{1}$ \\
$\text{RDB}_{1,2}$ & 3 & 1 & 1 & 32/32 & 8 & 16 & $\text{RDB}_{1,1}$\\

\hline
 & \textbf{k}  & \textbf{s} & \textbf{d}  & \textbf{p} &  \textbf{chns} &  \textbf{input} &   &  \\
	\hline  
	
$\text{conv1x1}_{1}$  & 1 & 1 & 1 & 0 & 32/64 & $\text{RDB}_{1,2}$ \\
$\text{Pool}_{2}$ & 2 & 1 & - & 0 & 64/64 & $\text{conv1x1}_{1}$ \\

\hline

& \textbf{k}  &  \textbf{s} &  \textbf{d}  &   \textbf{chns} &   \textbf{n-l} &   \textbf{g-r} &   \textbf{input} \\
\hline

$\text{RDB}_{2,1}$ & 3 & 1 & 1 & 64/64 & 8 & 16 & $\text{Pool}_{2}$ \\
$\text{RDB}_{2,2}$ & 3 & 1 & 1 & 64/64 & 8 & 16 & $\text{RDB}_{2,1}$\\


\hline
 & \textbf{k}  & \textbf{s} & \textbf{d}  & \textbf{p} &  \textbf{chns} &  \textbf{input} &   &  \\
	\hline  
	
$\text{conv1x1}_{2}$ & 1 & 1 & - & 0 & 64/128 & $\text{RDB}_{2,2}$ \\
$\text{Pool}_{3}$ & 2 & 1 & - & 0 & 128/128 & $\text{conv1x1}_{2}$ \\
\hline


& \textbf{k}  &  \textbf{s} &  \textbf{d}  &   \textbf{chns} &   \textbf{n-l} &   \textbf{g-r} &   \textbf{input} \\
\hline

$\text{RDB}_{3,1}$ & 3 & 1 & 1 & 128/128 & 8 & 16 & $\text{Pool}_{3}$ \\
$\text{RDB}_{3,2}$ & 3 & 1 & 1 & 128/128 & 8 & 16 & $\text{RDB}_{3,1}$\\

\hline
 & \textbf{k}  & \textbf{s} & \textbf{d}  & \textbf{p} &  \textbf{chns} &  \textbf{input} &   &  \\
	\hline  
	
$\text{conv1x1}_{3}$ & 1 & 1 & - & 0 & 128/256 & $\text{RDB}_{3,2}$ \\
$\text{Pool}_{4}$ & 2 & 1 & - & 0 & 256/256 & $\text{conv1x1}_{3}$ \\
\hline
%---------------------------------------------------------

& \textbf{k}  &  \textbf{s} &  \textbf{d}  &   \textbf{chns} &   \textbf{n-l} &   \textbf{g-r} &   \textbf{input} \\
\hline

$\text{RDB}_{4,1}$ & 3 & 1 & 1 & 128/128 & 8 & 16 & $\text{Pool}_{4}$ \\
$\text{RDB}_{4,2}$ & 3 & 1 & 1 & 128/128 & 8 & 16 & $\text{RDB}_{4,1}$\\

\hline
 & \textbf{k}  & \textbf{s} & \textbf{d}  & \textbf{p} &  \textbf{chns} &  \textbf{input} &   &  \\
	\hline  
	
$\text{conv1x1}_{4}$ & 1 & 1 & - & 0 & 128/256 & $\text{RDB}_{4,2}$ \\
AdaptiveAvgPool & - & - & - & - & 256/256 & $\text{conv1x1}_{4}$  \\
\hline
% ---------------------------------------------------------
 & \textbf{k}  & \textbf{s} & \textbf{d}  & \textbf{p} &  \textbf{chns} &  \textbf{input} &   &  \\
\hline  

$\text{conv1x1}_{5}$ & 1 & 1 & - & 1 & 256/128 & AdaptiveAvgPool \\
$\text{conv1x1}_{6}$  & 1 & 1 & - & 1 & 128/64 & $\delta$($\text{conv1x1}_{5}$) \\
$\text{conv1x1}_{7}$  & 1 & 1 & - & 1 & 64/96 & $\delta$($\text{conv1x1}_{6}$) \\


\hline

\end{tabular}}
\label{tab:illum_net}
\end{table}


==> Tables/network_rendering.tex <==

\begin{table}
\centering
\caption{Our rendering network architecture. We use this architecture for \textbf{Rendering Module}. }\label{tab:renderingnet}
\resizebox{.35\textwidth}{!}{%

\begin{tabular}{ l  c c c c c c c c }

\hline
Layers & \multicolumn{8}{c}{Parameters}  \\ 

% ---------------------------------------------------------
\hline
 & \textbf{k}  & \textbf{s} & \textbf{d}  & \textbf{p} &  \textbf{chns} &  \textbf{input} &   &  \\
\hline  

$\text{conv3x3}_{1}$ & 3 & 1 & 1 & 1 & 22/16 & $X$ \\
$\text{conv3x3}_{2}$ & 3 & 1 & 1 & 1 & 16/24 & $\delta$($\text{conv3x3}_{1}$) \\
$\text{conv3x3}_{3}$ & 3 & 1 & 1 & 1 & 24/24 & $\delta$($\text{conv3x3}_{2}$)\\
$\text{conv3x3}_{4}$ & 3 & 1 & 1 & 1 & 24/16 & $\delta$($\text{conv3x3}_{3}$) \\
$\text{conv3x3}_{5}$ & 3 & 1 & 1 & 1 & 16/3 & 
$\delta$($\text{conv3x3}_{4}$)\\


\hline

\end{tabular}}


\end{table}


==> Tables/network_shading.tex <==

\begin{table}
\centering

\caption{Our default U-Net based network architecture. We use this architecture for both the \textbf{Shading Module} and  \textbf{Albedo Estimation Module}. Here, \textbf{k} is the kernel size,  \textbf{s} the stride,  \textbf{d} the kernel dilation,  \textbf{p} the image
padding.  \textbf{chns} and  \textbf{input} are the number of input/output channels and the input to the layer. For RDBs and the GAB,  \textbf{n-l} is the number of layers,  \textbf{g-r} is the growth rate,  \textbf{e-s} is the embedding size,  \textbf{n-h} is the number of head and  \textbf{i-r} is the internal representation size. $\delta$ denotes rectified linear activation function. Note that the GAB is only used in the \textbf{Shading Module}.}

\resizebox{.45\textwidth}{!}{%
\begin{tabular}{ l  c c c c c c c c }

\hline
Layers & \multicolumn{8}{c}{Parameters}  \\ 
\hline


  & \textbf{k}  & \textbf{s} & \textbf{d}  & \textbf{p} &  \textbf{chns} &  \textbf{input} &   &  \\
	\hline
	
$\text{conv3x3}_{1}$ & 3 & 1 & 1 & 1 & 4/32 & $I_{in}$ \\
$\text{conv3x3}_{2}$ & 3 & 1 & 1 & 1 & 32/32 & $\delta$($\text{conv3x3}_{1}$) \\
$\text{Pool}_1$ & 2 & 1 & - & 0 & 32/32 & $\delta$($\text{conv3x3}_{2}$) \\
\hline

& \textbf{k}  &  \textbf{s} & d  &   \textbf{chns} &   \textbf{n-l} &   \textbf{g-r} &   \textbf{input} \\
\hline

$\text{RDB}_{1,1}$ & 3 & 1 & 1 & 32/32 & 8 & 16 & $\text{Pool}_1$ \\
$\text{RDB}_{1,2}$ & 3 & 1 & 1 & 32/32 & 8 & 16 & $\text{RDB}_{1,1}$\\

\hline
 & \textbf{k}  & \textbf{s} & \textbf{d}  & \textbf{p} &  \textbf{chns} &  \textbf{input} &   &  \\
	\hline  
	
$\text{conv1x1}_{1}$  & 1 & 1 & 1 & 0 & 32/64 & $\text{RDB}_{1,2}$ \\
$\text{Pool}_2$ & 2 & 1 & - & 0 & 64/64 & $\text{conv1x1}_{1}$ \\

\hline

& \textbf{k}  &  \textbf{s} &  \textbf{d}  &   \textbf{chns} &   \textbf{n-l} &   \textbf{g-r} &   \textbf{input} \\
\hline

$\text{RDB}_{2,1}$ & 3 & 1 & 1 & 64/64 & 8 & 16 & $\text{Pool}_2$ \\
$\text{RDB}_{2,2}$ & 3 & 1 & 1 & 64/64 & 8 & 16 & $\text{RDB}_{2,1}$\\


\hline
 & \textbf{k}  & \textbf{s} & \textbf{d}  & \textbf{p} &  \textbf{chns} &  \textbf{input} &   &  \\
	\hline  
	
$\text{conv1x1}_{2}$ & 1 & 1 & - & 0 & 64/128 & $\text{RDB}_{2,2}$ \\
$\text{Pool}_3$ & 2 & 1 & - & 0 & 128/128 & $\text{conv1x1}_{2}$ \\
\hline


& \textbf{k}  &  \textbf{s} &  \textbf{d}  &   \textbf{chns} &   \textbf{n-l} &   \textbf{g-r} &   \textbf{input} \\
\hline

$\text{RDB}_{3,1}$ & 3 & 1 & 1 & 128/128 & 8 & 16 & $\text{Pool}_3$ \\
$\text{RDB}_{3,2}$ & 3 & 1 & 1 & 128/128 & 8 & 16 & $\text{RDB}_{3,1}$\\

\hline
 & \textbf{k}  & \textbf{s} & \textbf{d}  & \textbf{p} &  \textbf{chns} &  \textbf{input} &   &  \\
	\hline  
	
$\text{conv1x1}_{3}$ & 1 & 1 & - & 0 & 128/256 & $\text{RDB}_{3,2}$ \\
$\text{Pool}_4$ & 2 & 1 & - & 0 & 256/256 & $\text{conv1x1}_{3}$ \\
\hline


& \textbf{e-s}  &  \textbf{n-l} &  \textbf{n-h}  &   \textbf{i-r} & \textbf{input}\\
\hline

GAB & 256 & 6 & 8 & 512 & $\text{Pool}_4$ \\
% ---------------------------------------------------------
\hline
 & \textbf{k}  & \textbf{s} & \textbf{d}  & \textbf{p} &  \textbf{chns} &  \textbf{input} &   &  \\
\hline  
	
$\text{conv3x3}_{3}$ & 3 & 1 & 1 & 1 & 256/128 & GAB \\
$\text{Up}_{1}$ & - & - & - & - & - &  $\text{conv3x3}_{3}$\\

$\text{conv1x1}_{4}$ & 1 & 1 & - & 0 & 512/256 & $\text{Up}_{1}$ + $\text{RDB}_{3,2}$ + $\text{RDB}_{3,1}$ \\

$\text{conv3x3}_{4}$ & 3 & 1 & 1 & 1 & 256/128 & $\delta$($\text{conv1x1}_{4}$) \\
$\text{Up}_{2}$ & - & - & - & - & - & $\delta$($\text{conv3x3}_{4}$) \\

$\text{conv1x1}_{5}$ & 1 & 1 & - & 0 & 256/128 & $\text{Up}_{2}$ + $\text{RDB}_{2,2}$ + $\text{RDB}_{2,1}$ \\

$\text{conv3x3}_{5}$ & 3 & 1 & 1 & 1 & 128/64 & $\delta$($\text{conv1x1}_{5}$) \\
$\text{Up}_{3}$ & - & - & - & - & - &  $\delta$($\text{conv3x3}_{5}$)\\

$\text{conv1x1}_{6}$ & 1 & 1 & - & 0 & 128/64 & $\text{Up}_{3}$ + $\text{RDB}_{1,2}$ + $\text{RDB}_{1,1}$ \\

$\text{conv3x3}_{6}$ & 3 & 1 & 1 & 1 & 64/32 & $\delta$($\text{conv1x1}_{6}$) \\
$\text{Up}_{4}$ & - & - & - & - & - & $\delta$($\text{conv3x3}_{6}$) \\

$\text{conv3x3}_{7}$ & 3 & 1 & 1 & 1 & 64/32 & $\text{Up}_{4}$ + $\text{conv3x3}_{2}$ \\
$\text{conv3x3}_{8}$ & 3 & 1 & 1 & 1 & 32/32 & $\delta$($\text{conv3x3}_{7}$) \\

\hline

\end{tabular}}



\label{tab:unet}
\end{table}

